SuperGlue: Learning Feature Matching with Graph Neural Networks

This paper introduces SuperGlue, a neural network that matches two sets of local features by jointly finding correspondences and rejecting non-matchable points. Assignments are estimated by solving a differentiable optimal transport problem, whose costs are predicted by a graph neural network. We introduce a flexible context aggregation mechanism based on attention, enabling SuperGlue to reason about the underlying 3D scene and feature assignments jointly. Compared to traditional, hand-designed heuristics, our technique learns priors over geometric transformations and regularities of the 3D world through end-to-end training from image pairs. SuperGlue outperforms other learned approaches and achieves state-of-the-art results on the task of pose estimation in challenging real-world indoor and outdoor environments. The proposed method performs matching in real-time on a modern GPU and can be readily integrated into modern SfM or SLAM systems. The code and trained weights are publicly available at https://github.com/magicleap/SuperGluePretrainedNetwork.

==> tables/megadepth.tex <==
\setlength\tabcolsep{4.0pt}
\begin{tabular}{llccccc}
    \toprule
    \multirow{2}{1cm}[-.4em]{Local features} & \multirow{2}{*}[-.4em]{Matcher}
    & \multicolumn{3}{c}{Pose estimation AUC} & \multirow{2}{*}[-.4em]{P} & \multirow{2}{*}[-.4em]{MS} \\
    \cmidrule(lr){3-5}
    && @5\degree & @10\degree & @20\degree & & \\
    \midrule
    \multirow{1}{*}{ContextDesc}
    & NN + ratio test & 41.13 & 55.59 & 67.32 & 71.7 & \06.1 \\
    \midrule
    \multirow{4}{*}{SIFT}
    & NN + ratio test & 31.55 & 43.65 & 56.11 & 63.1 & \03.8 \\
    & NN + OANet & 28.74 & 42.87 & 56.61 & 61.3 & 11.0\\
    & NN + NG-RANSAC & 33.69 & 45.91 & 58.36 & 86.9 & \04.3\\
    & \b{SuperGlue} & {\color{red}30.46} & {\color{red}43.29} & {\color{red}56.17} & {\color{red}84.0} & {\color{red}15.72}\\
    \midrule
    \multirow{4}{*}{SuperPoint}
    & NN + mutual & 24.00 & 34.86 & 46.32 & 39.1 & 10.7\\
    & NN + GMS & 30.02 & 41.24 & 51.10 & 60.8 & 10.7\\
    & NN + OANet & 35.68 & 48.72 & 60.57 & 71.5 & 19.2\\
    & \b{SuperGlue} & \b{47.01} & \b{61.99} & \b{74.14} & \b{93.8} & \b{25.3}\\
    \bottomrule
\end{tabular}
